Advancing Mathematical Epidemic Modeling via synergies with Chemical Reaction Network Theory and Lagrange-Hamilton Geometry

This essay reviews some key concepts in mathematical epidemiology and examines the intersection of this field with related scientific disciplines, such as chemical reaction network theory and Lagrange-Hamilton geometry. Through a synthesis of theoretical insights and practical perspectives, we underscore the significance of essentially non-negative kinetic systems in the development and implementation of robust epidemiological models. Our purpose is to make the case that currently mathematical modeling of epidemiology is focusing too much on simple particular cases, and maybe not enough on more complex models, whose challenges would require cooperation with scientific computing experts and with researchers in the "sister disciplines" involving essentially nonnegative kinetic systems (like virology, ecology, chemical reaction networks, population dynamics, etc).

==> BTJ1.tex <==
 \section{The importance of scientific computing: obtaining Bogdanov-Takens bifurcations by using symbolic algebra}\la{s:Gro}

 Symbolic stability and bifurcation analysis are very time consuming, since they require identifying  varieties like traces, determinants and Hurwitz determinants, evaluated at all the fixed points. It is plausible however that the equation satisfied by the union over the fixed points (i.e. the product of all the  respective equations), ends up simpler symbolically.


  We turn now to  some symbolic objects which we have introduced, and were not able to find  in the previous dynamical systems literature.

  \beD \la{d:E} The  determinant, trace, and Hurwitz determinant  of an algebraic system with respect to a subset of its solutions $A$ is defined by  the expressions

 \begin{equation}\label{dt} \bc detE=\prod_{i \in A} Det(J(E_i))\\ trE=\prod_{i \in A} Tr(J(E_i))\\H_{n,E}=\prod_{i \in A} H_n(E_i).\ec\end{equation}
 \eeD

  \beR \BEN \im Two choices of $A$ are of special interest: one, involving the product of the traces over all the fixed points, is useful for general dynamical systems. Another one, involving only the product  over  the interior points, is the one we used mostly, since eliminating the DFE from the study is advantageous computationally, and anyway the DFE is easy to study separately.

  \im  The varieties corresponding to $detE,trE$, etc, are the union of the varieties for each branch.  Due to the Vieta relations between the roots, they are expected to be considerably simpler than the individual expressions for the various branches.

  \im Interestingly, $detE,trE$, etc seem related up to proportionality  to the results obtained  via the  GroebnerBasis elimination command

 \begin{equation}\label{Gdt}\bc {detG}=\text{GroebnerBasis}[Numerator[Together[[\{\text{dyn}[[1]],\text{dyn}[[2]], Det(X) \}]],\text{par},X]\\{trG}=\text{GroebnerBasis}[Numerator[Together[[\{\text{dyn}[[1]],\text{dyn}[[2]], Tr(X) \}]],\text{par},X]\ec,\end{equation}
 which are easily obtained via the script:
\begin{verbatim}
 GBH[mod_,scal_,cn_ : {}] :=
     GroebnerBasis
     [Numerator[Together[[Join[ mod[[1]], {scal}]]],
     mod[[3]],  mod[[2]]]
\end{verbatim}
(recall that mod=\{dyn,var,par\}).
  To use this in two dimensions it is enough to apply it with scal= trace and scal=determinant.
  \iffalse
 \begin{verbatim}
 jacJ = JTDP[model, \[Zeta]][[1]] // FullSimplify;
    trJ = Tr[jacJ];
    detJ= Det[jacJ];
    Print[" detG is ", detG = GBH[mode, detJ][[1]] // FullSimplify]
    Print[" trG is", trG = GBH[mode, trJ][[1]] // FullSimplify]
    eq = Join[Thread[{trG, detG} == 0], Thread[model[[3]] > 0]];
Timing[re = Reduce[eq] // FullSimplify]
\end{verbatim}
\fi


\EEN

\eeR


\beR \la{r:easy} \BEN \im The computation of candidates for the Bogdanov-Takens bifurcations for all the fixed points in two dimensions
 may be achieved via the single command\\
 {
 \begin{equation}\label{Easy} Reduce[\{trG == 0, detG == 0,cp\}],\end{equation}
 where cp are positivity and other eventual constraints on the variables and parameters.
}



\im In more dimensions, it is enough a priori to replace the trace in \eqr{Easy} by the maximal
 dimension Hurwitz determinant.

 \EEN
 \eeR



==> Jin.tex <==


\sec{Particular case: a three dimensional generalization with $\g_s \ge 0, \de \ge 0$ of the model of  \cite{Jin} \la{s:Jin}}

By assuming $\b_r=i_s=0, \b_s=\b$ in \eqr{sirP}, and $\de_q=0$ (i.e. by ignoring the quadratic terms which appeared via the normalization), we arrive at a dynamical system with eight parameters $\left\{b,\beta ,\gamma ,\gamma _r ,\mu ,\xi,\gamma _s,\delta \right\}$, which contains two parameters $\g_s \ge 0, \de \ge 0$ more than \cite{Jin}. Putting $d_1=i_r +\delta +\mu,d_s=\ga_r+\mu,d_r=\ga_r+\mu$, the number of parameters is reduced to $7$:

\be{JMG}
\bc
\i'(t)= \i(t)\pr{\b \s(t) (1+\xi \i(t))-d_i},\\
\s'(t)=b -\b \s(t) \i(t) (1+\xi \i(t))+\g_r \r(t)-d_s \s(t),\\
\r'(t)=\g \i(t)+\g_s \s(t)-d_r \r(t).
\ec
\ee


\beR
The first generalization $\g_s \ge 0$ is minor, it only increases the time of execution of certain quantities.  Including an extra-death rate $\de$ is more substantial, since  assuming $\de=0$ makes \cite{Jin}'s problem  essentially two-dimensional, while \eqr{JMG} isn't. We  note here that a huge proportion of the related mathematical epidemiology literature contains models
which are essentially two-dimensional, due to assumptions like $\de=0$, or $\ga_r=0,$ which are not fully justified from the epidemiological point of view.
\eeR

\ssec{Further calculations for the generalized \cite{Jin} model}
\BEN
\im As noted already, the system \eqr{JMG}  has at most two endemic points, whose
  $\i$ coordinate satisfies a second order equation
  {\be{qi}\bc A i^2+ B i + C =0\\A= \beta  \xi  \left(\gamma  \mu +(\delta +\mu ) d_r \right)>0\\B=\beta \left( d_r (\delta +\mu-b \xi )+\gamma  \mu \right)\\C=d_i \mu(d_r+\g_s)\pr{1-\mR_0}=- det_{DFE}.
 \ec\ee}
 This checks with \cite[(2.2)]{Jin} when $\g_s=\de=0$.




\im The discriminant $\D=B^2-4AC$ \sats
 \be{DJin}
\fr \D \beta =\beta  \left(d_r (b \xi +\delta +\mu )+\gamma  \mu \right){}^2-4 \mu  \xi  d_i \left(\gamma  \mu +(\delta +\mu ) d_r\right) \left(d_r+\gamma _s\right)
\ee
 and is positive iff\fn[5]{the result checks with \cite[pg. 484-485]{Jin}, after some  substitutions like $\xi ->A p,$ etc}
 \be{beD}\b >\b_d=\frac{4 \mu  \xi  d_i \left(d_r+\gamma _s\right) \left(\gamma  \mu +(\delta +\mu ) d_r\right) }{\left(d_r (b \xi +\delta +\mu )+\gamma  \mu \right){}^2}.\ee


 %Note that \eqr{DJin} allows explicitizing the extra parameter $\g_s$ along the curve $\D=0$.
 \im {The equation $\i'/\i=0$ yields $s=\frac{d_i }{\beta  (i \xi +1)}>0.$ \Fr $r=\frac{\gamma  i+\gamma _s s}{\mu +\gamma _r}$.
Thus, a positive $i$ yields always an endemic point. }

\EEN



 We will order the two possible endemic points $E_1,E_2$ by their $i$ coordinates, given by
 $ i_1= \frac{-B-\sqrt{\Delta}}{2A}  \; \mbox{and} \quad i_2= \frac{-B+\sqrt{\Delta}}{2A}.$

 \beR Note that when $C = 0\Eq \mR_0=1$ we have $ i_1=0, i_2= -\frac{B}{A}$, which implies a transition in the number of  endemic points when crossing this boundary.
 \eeR

A major part of  \cite{Jin} is dedicated to bifurcation diagrams which demonstrate the presence of Hopf and Bogdanov-Takens bifurcations. We will review briefly these concepts in the next section. 

==> Mogh.tex <==

\subsection{One dimensional bifurcation diagram in the case $ \beta_ 0 < \beta_ 2 %\g_s=0, \delta>0
$}

We exemplify this case using the   SIR model of  \cite{Mogh} \eqr{sirM}.

\figu{bifM}{Bifurcation diagram \wrt\  $\b$ when $b = 1, \g= 1, \xi= 4, d= 1/4$ in \eqr{sirM}. In between $\beta_ d=0.226757 $ and $\beta_ 0=0.3125$ there exist three fixed points,  with $E_0$  stable and $E_1,E_2$ unstable. After   $\beta_ 0$ $E_1$ exits the domain, $E_0$  becomes unstable.  $E_2$  becomes stable after $\beta_ 2=0.331182$. In between $\beta_ 0,\beta_ 2$ there is no fixed stable point, and there  exists at least one stable cycle --{see Figure \ref{fig:spb2}}. At $ \beta_ 2$ and $\beta_ 1=0.267457$  the respective traces change sign.} {1}

\subsubsection{Bifurcation diagram of co-dimension two}

\figu{mapM}{Bifurcation diagram of co-dimension two for the system \eqr{sirM} with $b = 1, \xi= 4, d= 1/4$. The blue curve $Tr[J_2]=0$ contains Hopf candidates (for example, at  $ P_1= (0.298484,  0.943937), H=(0.2, 0.75),\beta_ 2=(0.331182,1),$  the eigenvalues of the Jacobian    at $E_2$ are \resp\ $\pm 0.541022 Im$, $ \pm 0.701516\; Im$ and $ \pm 0.745862 \; Im$). The  point $P_2=(0.0652696,  0.335786)$,  the intersection of the curve $Tr[J2]=0$ with $Dis=0=det[J2]$ is a Bogdanov-Takens candidate, with eigenvalues  at $E_2=E_1$ are $(0,0)$ .}{1.1}

\subsubsection{Time and phase plots at $ (\b=0.32 \in (\beta_ 0,\beta_ 2),  \g=1) $}
In the following figures, we provide time and phase plots at the point  $ (\b=0.32 \in (\beta_ 0,\beta_ 2),  \g=1) $:

\begin{figure}[H] %Mogh-jinT.nb
	\centering
	\begin{subfigure}[a]{0.31\textwidth}
		\includegraphics[width=\textwidth]{solb2}
		\caption{Plot of the dynamics in time with $t_f=400$ and $(s_0'',i_0'')=(1.3, 0.9)$,  indicating the existence of a limit cycle surrounding  $E_2=(1.208, 0.5584)$ \label{tR}.}
	\end{subfigure}
	~
	\begin{subfigure}[a]{0.31\textwidth}
		\includegraphics[width=\textwidth]{ptB}
		\caption{Time plot of $(s,i)$  with $t_f=600$ and $(s_0,i_0)=(1.7,0.6)$\label{tB}  .}
	\end{subfigure}
	~
	\begin{subfigure}[a]{0.31\textwidth}
		\includegraphics[width=\textwidth]{ptO}
		\caption{Time plot of $(s,i)$  with $t_f=500$ and   $(s_0',i_0')=(1.5,0.6)$ \label{tM} .}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.31\textwidth}
		\includegraphics[width=\textwidth]{spR}
		\caption{Phase plot corresponding to the time plot \ref{tR}, including a trajectory in violet starting outside the cycle.}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.31\textwidth}
		\includegraphics[width=\textwidth]{spB}
		\caption{Phase plot corresponding to the time plot \ref{tB}, including a trajectory  starting very close to the cycle.}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.31\textwidth}
		\includegraphics[width=\textwidth]{spO}
		\caption{Phase plot corresponding to the time plot \ref{tM}, including a trajectory starting inside the cycle.}
	\end{subfigure}
	~
	\begin{subfigure}[c]{0.48\textwidth}
		\includegraphics[width=\textwidth]{spf}
		\caption{$(s,i)$ phase plot. The fixed point $E_2$ is unstable with eigenvalues $0.01782\pm 0.711 Im$. The Floquet exponents of the cycle are $(-1.0331\times 10^{-7}, -0.0367982)$. The point $E_0=(4,0)$ is a saddle point with eigenvalues $(-0.25, 0.030)$ (and the fixed point $E_1$ is outside the domain).}
	\end{subfigure}
	\caption{Time and phase  plots at the point  $ (0.32,  1)$, with $\beta \in (\beta_ 0,\beta_ 2)$ --see also figure (\ref{f:bifM}).}
	\label{fig:spb2}
\end{figure}
 %Eco-Mogh-Jin.nb
	



==> crit.tex <==
\section{ A critic of the mathematical epidemiology bifurcations literature}\la{s:crit}

 We believe that a great part of the mathematical epidemiology literature  suffers today from two   draw-backs.
\BEN \im   The major one  is the lack of ``electronic reproducibility", i.e.  of  notebooks made public.
Here, we provide  electronic notebooks   for the papers cited above,  where the reader may  recover the results,  and also modify  them as he pleases, for analyzing similar models.
We believe that electronic  reproducibility in the above sense  should    be  the norm in the  field of mathematical biology.

 \im A  second draw-back in our opinion is too much focus  on simple particular  cases, furthermore studied under simplifying assumptions, which are  often  difficult to justify epidemiologically, like assuming $0$ deaths or eternal immunity. It seems sometimes  that  the   justification of the simplifying assumptions is to  allow a ``solution by hand", in the spirit of ``mathematics olympiad problems". Solving particular cases may of course be quite useful pedagogically, but is not efficient.  For just one of many examples where symbolic computing beats easily hand computations,
 note that the ``mathematics olympiad literature" restricts itself often to polynomials  of order $2$, to be able to use their elementary discriminant formula, which is of course unnecessary nowadays.
 We believe that mathematical epidemiology
 could be better served by relying more heavily on  modern symbolic computation. %As another benefit,  from this point of view  there is no need  to dedicate separate papers  to each  particular case  of general models like \eqr{Vys}.  A more natural approach   would be to study unified general cases symbolically as far as possible (until encountering time constraints),   pinpointing  how far can one push symbolics, and  turn to symbolic or  numeric particular cases only subsequently.

  
 \im Lots of papers in ME seem animated by an ambition to present computations  performed entirely by hand
 for low dimensional, few parameter examples, and make abstraction of the power of modern scientific  computing. No mention is being made of software which can perform the computations for higher dimensions, and  offers of making notebooks public are very rare. %This lengthens the papers and renders reading them very time consuming.

\blue{ An example of this is the excellent hand computations paper \cite{Jin}, discussed further below, which at its turn was motivated by adding information on Bogdanov-Takens bifurcations to a previous paper \cite{Mogh}. While the ``tour de force" of \cite{Jin} is impressive, their paper is not at all user friendly, and may be easily generalized by entrusting their computations to a CAS. We have illustrated these points by   entrusting the task to simple Mathematica scripts, which may be used in fact for any epidemiological model.}


\beR  We note that the Google search "mathematical epidemiology" "Groebner bases" produces currently very few resultsy. On the other hand, the Google search "bifurcations" "Groebner bases" produces more than 10 pages of results. This is rather surprising, given that most ME papers (if not all) deal with polynomial systems, for which Groebner bases are an essential tool, and that a lot of them deal with bifurcations. \eeR
\im Lack of knowledge of the literature of the parallel sister sciences. For example, most papers in ME start by dedicating a section to establishing the essential non-negativity and compactness of the system considered. However, this is usually unnecessary since  essential non-negativity for polynomial systems can be verified by ``eye inspection" via the very simple
 ``Hungarian lemma"  well-known in  the \CRN\ literature  \cite{hun},  \cite[Thm 6.27]{Toth} (see Lemma \ref{l:hun} below), which seems unknown to mathematical epidemiologists. %Note also that compactness is  trivial for papers which deal with systems that are mass conserving (i.e. live in a compact), or mass diminishing (due to extra deaths).

 \EEN

\iffalse
 For us, the hope for unification and progress may come from
the new discipline called {\bf algebraic/computational biology}
see  \cite{pachter2005algebraic,macauley2020case}, which  by its nature uses the practically universal language  of CAS's (Mathematica, Maple), and focuses on the  essential bottleneck:
the time-length of the computations.


  Mathematical epidemiologists have also invested lots of effort  in these directions.
We believe that  two
 methodological issues  impede  however the development of  this subfield of mathematical
 epidemiology: the exclusive concern with particular examples,
 and the insufficient use of symbolic scientific computing.

\fi

==> exa.tex <==


 We turn next to representing some examples of epidemic models as chemical reaction networks. We use the free software furnished by \cite{Toth}.
\BEN \im
The first, the three parameter  SIR model with demography of Hethcote, illustrates
the fact that with only one  ``susceptible" class (producing ``new infections"), and in the absence of epidemic deaths, which implies that the sums of the rates in the RHS's is 0 (and constant total population), epidemic models have only one interior fixed point. (Clearly, this is an immense mathematical simplification).
\im The second example illustrates both the fact that several susceptible classes destroy the uniqueness of the interior fixed point, and the fact that the proportions of a varying population model may sometimes, after algebraic manipulations, be brought to a form where the sums of the rates in the RHS's is 0.
\im The third example, due to \cite{Mogh,Jin}, is one of the simplest example displaying periodic orbits, and is  a close cousin of the autocatalator process of \CRN\ theory.
\iffalse
\im The fourth example illustrates  the fact that varying population models with at least four classes (SEIR, SAIR, etc) and even just one susceptible class, may already be so complicated  that they  are not yet fully understood, despite more than 40 years of research (especially in the case of several interior fixed points.\fn[4]{For that reason, their proportions are typically studied via ad-hoc or   heuristic approximations \cite{AABBGH,AABH,AAH}, which require  singular perturbation methods \cite{Kuehn} to be made rigorous.}

We have chosen here the SIRC/SIRW  epidemic model first introduced for studying influenza \cite{Casagrandi}, which is representative of the case when there are two susceptible classes, and the \DFE\ stability parameter $R_0$ is not explicit.
\fi
\EEN

 \ssec{The 0-sum SIR with one susceptible class and unique interior point} The  classic three parameter  SIR model with demography, but no  epidemic deaths of Hethcote is a 0-sum model, which may be represented as:
 \be{sirC}
 \bc \s'(t) = -  \beta  \s(t) \i(t)
    + \L\pp{1 - \s(t)}\\
\i'(t) =
 \i(t)\pp{\beta \s(t)  - \pr{\L +  \g }}\\
\r'(t) =  \g    \i(t)  -\L \r(t)\\ \s(t) + \i(t) + \r(t)=1\ec \Eq
\bc \s'(t) = -  \beta  \s(t) \i(t)
    + \L\pp{\i(t) + \r(t)}\\
\i'(t) =
 \i(t)\pp{\beta \s(t)  - \pr{\L +  \g }}\\
\r'(t) =  \g    \i(t)  -\L \r(t)\\ \s(t) + \i(t) + \r(t)=1\ec.
\ee

 The first form is ``open network". The second ``closed network" form has the following mass-action representation
 $$\bc  S+I ->2 I &\beta s i \\I->R &\g  \i\\
 I->S & \L \i \\ R->S &\L  \r\ec,$$
with  $n_V=5$ vertices, $n_R=4$  edges, rank 2
and 2 linkage classes.  The deficiency of the CRN is $\delta=n_V-rank(S)-n_C=5-2-2=1$.

Factoring the middle equation yields the stationary points $(1,0,0)$ (\DFE) and
$$E_*=\set{s_*=\fr{\L +  \g }\b,\pr{1-s_*} \fr{b } {\beta s_*},\pr{1-s_*} \pp{1-\fr{b } {\beta s_*}}}$$ (endemic point), which is in the domain  iff $$R_0 :=\fr\beta {\L +  \g }>1.$$

This model is essentially two-dimensional, and its coefficients are simple enough to ensure $Tr[Jac[E_*]]<0$,  and therefore does not allow Hopf bifurcation.

\red{In fact, the same is true for the
more general version in  \cite{AABH}, since the constraint $s+i+r=1$ forces the rank of the stoichiometric matrix to be at most $2$, and a minimum of 3 is necessary for Hopf bifurcation?}




Thus, to find Hopf bifurcations, one needs to go to four compartment models like SEIR \cite{li1995global}, SAIR\cite{ottaviano2021threshold,AABH}, SIRW\cite{Kuehn}, or to consider ``generalized SIR models" \cite{Mogh,Jin}, which are precisely crafted for this purpose, and less used  in applied epidemiology -- see subsection \ref{ex:MJ}.


\ssec{A 0-sum $(n=3,n_R=5,r=2)$ example with two susceptible classes S,R, and two interior points}
 The model
\be{sirFs}
\bc \s'(t) = -  (\beta  -\delta)\s(t) \i(t)
     + \L \pr{\i(t) + \r(t)}\\
\i'(t) =
 \i(t)\pp{(\b-\delta) \s(t) +(\beta_ r-\delta)  \r(t) - (\L +  \g )}\\
\r'(t) =-(\beta_ r-\delta) \i(t) \r(t)+\g    \i(t)  -\L \r(t)\ec
\ee

is a particular case of \eqr{sirF} below. We include this example despite the fact that it does not allow Hopf bifurcation, to draw the attention to a subtle point in epidemiology: the fact that a model which does include epidemic deaths at rate $\de$ may be isomorphic to a model which doesn't, by a relabeling of the parameters \cite{Nill}.

The reaction representation is $$\bc  S+I ->2 I &\beta \s \i\\I+R-> 2I &\beta_ r \r \i  \\I->R &\g  \i\\ I->S & \L \i \\ R->S &\L  \r\ec.$$
% S + I->2S+I &(\delta \s \i)\\2 I->3I &(\delta  \i^2)\\.$$
It has  $n_V=6$ vertices $I,R,S+I,S+R,2 I,S$ (the first $n_S=4$ of which are sources), $n_R=5$  edges,
and 2 linkage classes.  The deficiency of the CRN is $\delta=n_V-rank(S)-n_C=6-2-2=2$.

\figu{Hethbr}{}{.9}




\subsection{The \cite{Mogh,Jin} non 0-sum SIR models with superinfection \label{ex:MJ} } %,and the ``autocatalator SIR model" }

 The \cite{Jin} process, of type  $(4,7,4 )$, is  defined  by:
\be{sirJ}
\bc \s'(t) = \L - \m \s(t) - \beta (1+ \xi \i(t))\s(t) \i(t) +\g_r \r(t)
     \\
\i'(t) =
 \i(t)\pp{\beta (1+ \xi \i(t))\s(t) - (\m +  \g + \de )}\\
 \r'(t)=\g \i(t) -(\m +\g_r) \r(t)
\ec
\ee
\figu{Jin}{Interaction graph of system \eqr{sirJ}.% when $\delta=0$.
}{1.1}

The \cite{Mogh} process, of type $(3,5,3)$, is almost a particular case of \eqr{sirJ}, obtained when $\g_r=0$. In order to conform to the original In this case we may ignore at first the last equation and study the two-dimensional model:
\be{sirM}
\bc \s'(t) = \L - \m \s(t) -  (\b+ \beta_ \xi \i(t))\s(t) \i(t)
     \\
\i'(t) =
 \i(t)\pp{(\b+ \beta_ \xi  \i(t))\s(t) - (\m + \T \g )}\\
\ec, \; \T \g :=\g+\de, \beta_ \xi:=\beta \xi
\ee

The term $\beta_ \xi$ is interpretable in epidemiology as a ``superinfection" rate.

\beR In the particular case $\b=0, \mu=0,$ this process is ``one reaction away" from the famous autocatalor \cite{gray1986new,fercec2019limit}. In the notation of \cite[(60)]{Nagy}, putting $b=k_0, \beta_ \xi=k_1, \g=k_2$, and adding a second linear transfer of rate $\g_s=k_3$ from $\s$ to $\i$ yields the autocatalator. \eeR

\figu{Mogh}{Interaction graph of system \eqr{sirM}.}{1.1}




%\sssec{The  SIRC/SIRW  epidemic model}\la{ex:SIRC}


==> ni.tex <==
To simplify the notations, we rewrite this as:

\begin{align}
S'&=-\tilde{\ga}_s S+\tilde{\ga}_r R + \tilde{i}_s I -
\tilde{\b}_s(1+\tilde{\xi}_s)SI\\
R'&=-\tilde{\ga}_r R+\tilde{\ga}_s S + \tilde{i}_r I -
\tilde{\b}_r(1+\tilde{\xi}_r)RI\\
I'&=-\tilde{i}I+\tilde{\b}_s(1+\tilde{\xi}_s)SI+
\tilde{\b}_r(1+\tilde{\xi}_r)RI=:\tilde{i}I(X-1)
\end{align}

where we have put

\begin{align}
&\tilde{\ga}_s=\ga_s,\qquad\tilde{\ga}_r=\ga_r+b,\qquad
\tilde{i}_s=i_s+b,\qquad\tilde{i}_r=i_r,\qquad
\tilde{i}=\tilde{i}_s+\tilde{i}_r\\
&\tilde{\b}_s=\beta_ s-\delta,\qquad
\tilde{\b}_r=\beta_ r-\delta,\qquad
\tilde{\xi}_s=\xi\beta_ s/(\beta_ s-\delta),\qquad
\tilde{\xi}_r=\xi\beta_ r/(\beta_ r-\delta).\label{tilde_xi}
\end{align}

Now we may without loss fix time scale by putting $\tilde{i}=1$ leaving us with with a 7-parameter model. The case $\tilde{\xi}_s=\tilde{\xi}_r=0$ has been studied by \cite{Nil1}.



{\remark

The parameter change \eqref{tilde_xi}
$(\beta_ s,\beta_ r,\delta,\xi)\leftrightarrow(\tilde{\b}_s,\tilde{\b}_r,\tilde{\xi}_s,\tilde{\xi}_r)$ doesn't reduce the number of parameters, so it's a matter of taste which one to keep.}



